Auction-Based Scheduling

Many sequential decision-making tasks require satisfaction of multiple, partially contradictory objectives. Existing approaches are monolithic, namely all objectives are fulfilled using a single policy, which is a function that selects a sequence of actions. We present auction-based scheduling, a modular framework for multi-objective decision-making problems. Each objective is fulfilled using a separate policy, and the policies can be independently created, modified, and replaced. Understandably, different policies with conflicting goals may choose conflicting actions at a given time. In order to resolve conflicts, and compose policies, we employ a novel auction-based mechanism. We allocate a bounded budget to each policy, and at each step, the policies simultaneously bid from their available budgets for the privilege of being scheduled and choosing an action. Policies express their scheduling urgency using their bids and the bounded budgets ensure long-run scheduling fairness. We lay the foundations of auction-based scheduling using path planning problems on finite graphs with two temporal objectives. We present decentralized algorithms to synthesize a pair of policies, their initially allocated budgets, and bidding strategies. We consider three categories of decentralized synthesis problems, parameterized by the assumptions that the policies make on each other: (a) strong synthesis, with no assumptions and strongest guarantees, (b) assume-admissible synthesis, with weakest rationality assumptions, and (c) assume-guarantee synthesis, with explicit contract-based assumptions. For reachability objectives, we show that, surprisingly, decentralized assume-admissible synthesis is always possible when the out-degrees of all vertices are at most two.

==> bidding_games.tex <==
%!TEX root=main.tex

\section{Proof Sketch of Thm.~\ref{thm:RT-reach}}
\label{app:RT-reach}

\thmRTreach*
Fix a bidding game $\tup{\G,\spec}$ with the reachability objective $\spec = \reach_\G(\set{t})$ for the single target $t\in \V$. 
If the game starts at $t$, since the objective is already fulfilled---irrespective of the budget, hence $\th_\spec^\G(t)=0$.
For every other vertex $v$, it is known that the threshold can be represented as:
\begin{align}\label{eq:bidding games:reach threshold}
	\th_\spec^\G(v) = \frac{1}{2}\left( \th_\spec^\G(v^+) + \th_\spec^\G(v^-)\right),
\end{align} 
where $v^+$ and $v^-$ represent the successors of $v$ with the largest and the smallest thresholds, respectively.
Then if the initial configuration is $\tup{v,B} = \tup{v,\th_\spec^\G+\epsilon}$, for any given $\epsilon>0$, \PO can bid $\bidpol(v) = \sfrac{1}{2}(\th_\spec^\G(v^+) - \th_\spec^\G(v^-))$ and go to $\actpol(v) = v^-$ upon winning.
If he wins and moves the token to $v^-$, then his new budget will be $B - \bidpol(v) = \th_\spec^\G(v^-) + \epsilon$.
If he loses and \PT moves the token to a successor $v'$, then we know that \PT must have bid higher than $\bidpol(v)$ which \PO will receive, so that \PO's new budget will be at least $B + \bidpol(v) = \th_\spec^\G(v^+)+\epsilon$, larger than $\th_\spec^\G(v') + \epsilon$ by definition of $v^+$.
This way, the strategy $\tup{\actpol,\bidpol}$ can ensure that for every vertex $v'$ where the token may reach from $v$ in one step, the invariant $B>\th_\spec^\G(v')$ is maintained, so that \PO can win from $v'$, which can be repeated and eventually \PO will reach $t$. This strategy works on DAGs. For graphs with cycles, a little extra work on the bidding policy is needed to get out of cycles and move towards the target \cite{LLPSU99}.



==> motivating_examples.tex <==
%!TEX root=main.tex

\section{Illustrative Examples}
\label{sec:illustrative examples}
%
%Let us now go into more detail. 
%Concretely, we consider the path planning problem on a given finite graph $\G$ where the path needs to satisfy two given $\omega$-regular objectives $\spec_1$ and $\spec_2$, simultaneously. 
%We introduce \emph{tenders} as policies equipped with bidding capabilities, serving as the building blocks of auction-based scheduling. 
%A tender $\t_i$, with $i\in\set{1,2}$, for the objective $\spec_i$ is a triple $\tup{\actpol_i,\bidpol_i,\B_i}$, where $\actpol_i$ and $\bidpol_i$ are the \emph{action policy} and the \emph{bidding policy} that propose the next edge and the next bid within the available budget at each point in time, respectively, and $\B_i$ is a constant in $[0,1)$, called the \emph{threshold budget}, such that if the initial available budget for $\t_i$ is greater than $\B_i$ then $\spec_i$ is guaranteed to be fulfilled. 
%The \emph{composition} of $\t_1$ and $\t_2$, denoted $\comp{\t_1}{\t_2}$, is a policy in $\G$ augmented with a register to keep track of the available budgets; the composition works as follows. 
%Firstly, $\t_1$ and $\t_2$ are \emph{compatible} (for composition) only if $\B_1+\B_2<1$, because then we can distribute the total initial budget---normalized to $1$---between the two tenders in a way that they have more budgets than their thresholds.
%The current {\em configuration} is a pair $\zug{v, B_1}$, denoting the current vertex $v$ and the current budget $B_1$ available to the first tender. With the normalization of the total budget,  the available budget of the second tender is implicitly $B_2 = 1-B_1$. 
%The initial configuration is $\zug{\vinit, B^0_1}$ such that, for each $i \in \set{1,2}$, we have $\B_i <  B_i^0\leq 1$. 
%At each point in time, each bidding policy $\bidpol_i$ independently and concurrently chooses a bid $b_i \leq B_i$.
%Whoever bids higher wins the bidding, pays its bid to the other tender, and uses its action policy $\actpol_i$ to choose the next vertex $u_i$.
%%At each point in time, the tender $\t_i$ independently performs an {\em action} $\zug{u_i, b_i}$ (computed respectively by $\actpol_i$ and $\bidpol_i$), where $b_i \leq B_i$ is the bid and $u_i$ is the proposed next vertex. 
%%Whoever bids higher wins the bidding, pays its bid to the other tender, and its proposed next vertex is selected.
%Formally, if $b_1 \geq b_2$, the next configuration is $\zug{u_1, B_1 - b_1}$, and otherwise it is $\zug{u_2, B_1 + b_2}$. 
%The central problem studied in this paper is decentralized synthesis of tenders for auction-based scheduling:
%Given $\G$, $\spec_1$, and $\spec_2$, synthesize $\t_1$ such that for every $\t_2'$, the path generated by $\comp{\t_1}{\t_2'}$ satisfies $\spec_1$, and---\emph{independently}---synthesize $\t_2$ such that for every $\t_1'$, the path generated by $\comp{\t_1'}{\t_2}$ satisfies $\spec_2$.
%It follows that the path generated by $\comp{\t_1}{\t_2}$ satisfies $\spec_1\land\spec_2$.

\KM{Just copy+pasted from the previous section}
We consider three instantiations of decentralized synthesis based on the trade off between the strengths of the solutions and the strengths of the assumptions that the tenders make on each other:


\noindent{\bf Strong decentralized synthesis.}
Here, tenders make no assumptions on each other, thus the solutions provide the strongest (the most robust) guarantees.

\tikzset{%
glow/.style={%
preaction={#1, draw, line join=round, line width=0.5pt, opacity=0.04,
preaction={#1, draw, line join=round, line width=1.0pt, opacity=0.04,
preaction={#1, draw, line join=round, line width=1.5pt, opacity=0.04,
preaction={#1, draw, line join=round, line width=2.0pt, opacity=0.04,
preaction={#1, draw, line join=round, line width=2.5pt, opacity=0.04,
preaction={#1, draw, line join=round, line width=3.0pt, opacity=0.04,
preaction={#1, draw, line join=round, line width=3.5pt, opacity=0.04,
preaction={#1, draw, line join=round, line width=4.0pt, opacity=0.04,
preaction={#1, draw, line join=round, line width=4.5pt, opacity=0.04,
preaction={#1, draw, line join=round, line width=5.0pt, opacity=0.04,
preaction={#1, draw, line join=round, line width=5.5pt, opacity=0.04,
preaction={#1, draw, line join=round, line width=6.0pt, opacity=0.04,
}}}}}}}}}}}}}}
\tikzset{every state/.style={minimum size=0pt}}
\tikzset{%
target/.style={
preaction={#1, fill, opacity=0.5}
}}
\tikzset{cross/.style={
		preaction={#1, draw, cross out}}}
		



\begin{figure}
	\centering
	\begin{subfigure}[t]{0.3\textwidth}
		\centering
		\begin{tikzpicture}[node distance=0.7cm]
			\node[state,initial below]		(a)	at	(0,0)				{$a$};
			\node[state]		(b)	[left=of a]		{$b$};
			\node[state,target=blue]		(c)	[above=of b]		{$c$};
			\node[state,target=blue,target=red]		(d)	[below=of b]		{$d$};
			
			\node[state]		(e)	[right=of a]		{$e$};
			\node[state,target=red]		(f)	[above=of e]		{$f$};
			\node[state,target=blue]		(g)	[below=of e]		{$g$};
			
			\path[->,ultra thick]
				(a)		edge	[glow=blue]		(b)
				(b)		edge	[glow=red]		(d)
			;
						
			\path[->]
				(a)		edge		(e)
				(b)		edge			(c)
				(e)		edge	[glow=red]		(f)
						edge	[glow=blue]		(g);
		\end{tikzpicture}
		\caption{Strong}
		\label{fig:motivating example:robust}
	\end{subfigure}
	\begin{subfigure}[t]{0.3\textwidth}
		\centering
		\begin{tikzpicture}[node distance=0.7cm]
			\node[state,initial below]		(a)	at	(0,0)				{$a$};
			\node[state]		(b)	[left=of a]		{$b$};
			\node[state]		(c)	[above=of b]		{$c$};
			\node[state,target=blue,target=red]		(d)	[below=of b]		{$d$};
			
			\node[state]		(e)	[right=of a]		{$e$};
			\node[state,target=red]		(f)	[above=of e]		{$f$};
			\node[state,target=blue]		(g)	[below=of e]		{$g$};
			
			\path[->,ultra thick]
				(a)		edge	[glow=blue,glow=red]		(b)
				(b)		edge	[glow=red,glow=blue]		(d)
			;
						
			\path[->]
				(a)		edge		(e)
				(b)		edge			(c)
				(e)		edge	[glow=red]		(f)
						edge	[glow=blue]		(g);
		\end{tikzpicture}
		\caption{Assume-admissible}
		\label{fig:motivating example:admissible}
	\end{subfigure}
	\begin{subfigure}[t]{0.3\textwidth}
		\centering
		\begin{tikzpicture}[node distance=0.7cm]
			\node[state,initial below]		(a)	at	(0,0)				{$a$};
			\node[state]		(b)	[left=of a]		{$b$};
			\node[state,target=blue]		(c)	[above=of b]		{$c$};
			\node[state,target=blue,target=red]		(d)	[below=of b]		{$d$};
			
			\node[state]		(e)	[right=of a]		{$e$};
			\node[state,target=red]		(f)	[above=of e]		{$f$};
			\node[state,target=blue]		(g)	[below=of e]		{$g$};
			
			\path[->,ultra thick]
				(a)		edge	[glow=blue,glow=red]		(b)
				(b)		edge	[glow=red,glow=blue]		(d)
			;
						
			\path[->]
				(a)		edge		(e)
				(b)		edge			(c)
						edge		(f)
				(e)		edge	[glow=red]		(f)
						edge	[glow=blue]		(g);
		\end{tikzpicture}
		\caption{Assume-guarantee}
		\label{fig:motivating example:contract}
	\end{subfigure}
	\caption{Graphs with two reachability objectives given by targets: $T_\blue$, depicted in blue, $T_\red$ depicted in red, and $T_\blue \cap T_\red$ depicted in purple. The action policies of the red and blue tenders choose edges with, respectively,  red and blue shadows (shared edges in purple). If no edges from a vertex have red or blue shadow, then the respective tender is indifferent about the choice made. Thick edges depict the paths taken by the compositions of tenders.}
	\label{fig:motivating example}
\end{figure}
\begin{example}\label{ex:motivation:strong}
Consider the graph depicted in Fig.~\ref{fig:motivating example:robust} with a pair of {\em reachability} objectives having the targets $T_{\blue} = \set{c,d,g}$ and $T_{\red}=\set{d,f}$, respectively.  Their intersection $\set{d}$ is depicted in purple.
We present a pair of robust tenders $\t_{\blue}$ and $\t_{\red}$ with $\B_{\blue} = \sfrac{1}{4}$ and $\B_{\red}=\sfrac{1}{2}$, so that $\t_{\blue}$ and ${\t_{\red}}$ are compatible. We will show that $\t_{\blue}$ guarantees that no matter which compatible tender it is composed with, eventually $T_{\blue}$ is reached, and similarly $\t_{\red}$ ensures that $T_{\red}$ is reached. Therefore, $\comp{\t_{\blue}}{\t_{\red}}$ ensures that $d$ is reached.

We first describe $\t_{\blue}$. Consider an initial configuration $\zug{a, \sfrac{1}{4} + \epsilon}$, for any $\epsilon > 0$. Note that the other tender's budget is $\sfrac{3}{4}-\epsilon$. The first action of $\t_\blue$ is $\zug{b, \sfrac{1}{4}}$. There are two possibilities. First, $\t_{\blue}$ wins the bidding, then we reach the configuration $\zug{b, \epsilon}$, and since both successors of $b$ are in $T_{\blue}$, the objective is satisfied in the next step. Second, $\t_{\blue}$ loses the bidding, meaning that the other tender bids at least $\sfrac{1}{4}$, and in the worst case, we proceed to the configuration $\zug{e, \sfrac{1}{2}+\epsilon}$. Next, $\t_\blue$ chooses $\zug{g, \sfrac{1}{2}}$ and necessraily wins as $\t_\red$'s budget is only $\sfrac{1}{2} - \epsilon$, and we reach $g \in T_{\blue}$. We stress that $\t_\blue$ can be entirely oblivious about $\t_\red$, except for the implicit knowledge of $\t_\red$'s budget.

We describe $\t_{\red}$. Consider an initial configuration $\zug{a, \sfrac{1}{2} + \epsilon}$, for any $\epsilon > 0$. 
Initially, $\t_{\red}$ bids $0$, because it does not have a preference between going left or right. In the worst case, the budget stays $\sfrac{1}{2} + \epsilon$ in the next turn. 
Since both $b$ and $e$ have single successors in $T_{\red}$, thus $\t_\red$ must win the bidding. It does so by bidding $\sfrac{1}{2}$, which exceeds the available budget $\sfrac{1}{2}-\epsilon$ of $\t_\red$.\hfill$\triangle$
\end{example}

We now use the same problem as in Ex.~\ref{ex:motivation:strong}, and show that the conventional turn-based interaction may fail to fulfill both objectives.

\new{
\begin{example}\label{ex:turn-based fails}
	Consider again the graph depicted in Fig.~\ref{fig:motivating example:robust} with the targets $T_{\blue} = \set{c,d,g}$ and $T_{\red}=\set{d,f}$.
	Suppose $\actpol_\blue$ and $\actpol_\red$ are the two respective action policies, and we arbitrarily decide to make their interaction turn-based, where $\actpol_\red$ chooses actions in $a$ and $\actpol_\blue$ chooses actions in $b$ and $e$.
	It is clear that no matter which edge $\actpol_\red$ chooses from $a$, it cannot guarantee satisfaction of $T_\red$, because $\actpol_\blue$ can take the game to $c$ or $g$ depending on $\actpol_\red$'s choice.
	To overcome this, one could use contract-based synchronization protocols~\cite{majumdar2020assume} between $\actpol_\red$ and $\actpol_\blue$.
	However, tenders obtained using our strong synthesis approach can fulfill both objectives by natural means and without relying on any contracts.
	\hfill$\triangle$
\end{example}
}


Our algorithms for decentralized synthesis internally solve zero-sum {\em bidding games}~\cite{LLPU96,LLPSU99}. 
A bidding game is played on a finite graph by two players called \PO and \PT. 
The game proceeds as follows. The players have bounded budgets, and in each turn, both players bid for the right to take an action. 
A {\em strategy} in a bidding game, 
using our terminology, is a pair $\zug{\actpol, \bidpol}$ of action and bidding policies. The central question is to find a {\em winning strategy}, namely a strategy that guarantees winning, with respect to a given objective, no matter which strategy the opponent follows. 
For $\omega$-regular objectives, it is known~\cite{LLPU96,LLPSU99,AHC19} that each vertex $v$ 
can be associated with a {\em threshold} $\th(v)$ such that when \PO's budget at $v$ is $B_X > \th(v)$, \PO has a winning strategy, and when $B_X < \th(v)$, \PT has a winning strategy. 


Our algorithm to solve strong decentralized synthesis proceeds as follows. 
Given a graph $\G$ with an initial vertex $\vinit$ and two objectives $\spec_1$ and $\spec_2$, we solve two zero-sum bidding games $\G_1$ and $\G_2$, independently. Both games are played on the graph $\G$. In $\G_1$, \PO's objective is $\spec_1$ and in $\G_2$, his objective is $\spec_2$. 
Let $\th_1(\vinit)$ and $\th_2(\vinit)$ respectively denote the thresholds at $\vinit$ in $\G_1$ and $\G_2$. We show that a pair of robust tenders exist iff $\th_1(\vinit)+\th_2(\vinit)<1$. When they exist, for $i \in \set{1,2}$, we output the tender $\t_i = \zug{\actpol_i, \bidpol_i, \th_i(\vinit)}$, where the pair $\zug{\actpol_i, \bidpol_i}$ is a winning \PO strategy in the game $\G_i$. Since $\t_i$ is a winning strategy, it ensures that objective $\spec_i$ is satisfied when composed with {\em any} compatible strategy. Thus, necessarily, the composition $\comp{\t_1}{\t_2}$ of two tenders in $\G$ ensures that both objectives are satisfied!


\noindent{\bf Assume-admissible decentralized synthesis.}
While the guarantees of strong decentralized synthesis are appealing, it often fails as each tender makes the pessimistic assumption that the other tender can behave arbitrarily---even adversarially. 
We consider \emph{admissibility}~\cite{brenguier2015assume} as a stronger assumption based on rationality, ensuring compatible tenders to exist even when strong synthesis may fail. We illustrate the idea in the following example. 



\begin{example}\label{ex:motivation:assume-admissible}
Consider the graph in Fig.~\ref{fig:motivating example:admissible}, with reachability objectives given by targets $T_{\blue}=\set{d,g}$ and $T_{\red}=\set{d,f}$.
We argue that strong decentralized synthesis is not possible. Indeed, using the same reasoning for $\t_\red$ in Ex.~\ref{ex:motivation:strong}, we have $\th_\blue(a) = \th_\red(a) = 0.5$. 
On the other hand, observe that when synthesizing $\t_\red$, since $c \notin T_\blue$, we know that a  ``rational''  $\t_\blue$---formally, {\em admissible} $\t_\blue$ (see Sec.~\ref{sec:assume-admissible})---will not proceed from $b$ to $c$, and we can omit the edge. In turn, the threshold in $a$ decreases to $\sfrac{1}{4}$ for both objectives. Since the sum of thresholds is now less than $1$, two compatible tenders can be obtained. \hfill$\triangle$
\end{example}

In general, we seek an {\em admissible-winning tender}, which ensures that its objective is satisfied when composed with any admissible tender. 
Admissible-winning tenders are modular because they can be reused provided that the set of admissible actions of the other tender remains unchanged. 
For example, even when vertex $g$ is added to the red target set, the blue tender can be used with no change. Somewhat surprisingly, we show that in graphs in which all vertices have out-degree at most $2$, assume-admissible decentralized synthesis is always possible, and a pair of admissible-winning tenders can be found in PTIME. 



\noindent{\bf Assume-guarantee decentralized synthesis.}
Sometimes, even the admissibility assumption is too weak, and we need more direct synchronization of the tenders.
We consider assume-guarantee decentralized synthesis, where each tender needs to respect a pre-specified \emph{contract}, and as a result, their composition satisfies both objectives. We illustrate the idea below. 

\begin{example}\label{ex:motivation:assume-guarantee}
Consider the graph depicted in Fig.~\ref{fig:motivating example:contract}, with reachability objectives given by targets $T_{\blue}=\set{c,d,g}$ and $T_{\red}=\set{d,f}$. 
Here, the strong decentralized synthesis fails due to reasons similar to Ex.~\ref{ex:motivation:assume-admissible}.
The assume-admissible decentralized synthesis fails because from $e$, both objectives cannot be fulfilled, and from $b$, no matter which tender wins the bidding can use an admissible edge that violates the other objective (e.g., $(b,c)$ is admissible for $\t_\blue$ but violates $T_\red$).
We consider the {\em contract} $\tup{G_{\blue},G_{\red}}=\tup{\always\,\lnot c,\always\,\lnot f}$, which is satisfied when (a)~if $\actpol_{\blue}$ fulfills $G_{\blue}$, then $\actpol_{\red}$ fulfills $G_{\red}$, and 
(b)~if $\actpol_{\red}$ fulfills $G_{\red}$, then $\actpol_{\blue}$ fulfills $G_{\blue}$.
Now whichever tender wins the bidding at $b$ needs to fulfill its guarantee, because it cannot judge from the past interaction if the other tender fulfills its guarantee.
Therefore, from $b$, the next vertex will be $d$ under the contract, and using the same tenders from Ex.~\ref{ex:motivation:assume-admissible}, both objectives will be fulfilled.
\end{example}




